Embodied-R1: Reinforced Embodied Reasoning for General Robotic Manipulation

Generalization in embodied AI is hindered by the "seeing-to-doing gap," which stems from data scarcity and embodiment heterogeneity. To address this, we pioneer "pointing" as a unified, embodiment-agnostic intermediate representation, defining four core embodied pointing abilities that bridge high-level vision-language comprehension with low-level action primitives. We introduce Embodied-R1, a 3B Vision-Language Model (VLM) specifically designed for embodied reasoning and pointing. We use a wide range of embodied and general visual reasoning datasets as sources to construct a large-scale dataset, Embodied-Points-200K, which supports key embodied pointing capabilities. We then train Embodied-R1 using a two-stage Reinforced Fine-tuning (RFT) curriculum with a specialized multi-task reward design. Embodied-R1 achieves state-of-the-art performance on 11 embodied spatial and pointing benchmarks. Critically, it demonstrates robust zero-shot generalization by achieving a 56.2% success rate in the SIMPLEREnv and 87.5% across 8 real-world XArm tasks without any task-specific fine-tuning, representing a 62% improvement over strong baselines. Furthermore, the model exhibits high robustness against diverse visual disturbances. Our work shows that a pointing-centric representation, combined with an RFT training paradigm, offers an effective and generalizable pathway to closing the perception-action gap in robotics.

==> sections/abstract.tex <==
\begin{abstract}
% Generalization in embodied AI is hindered by the ``seeing-to-doing gap'', stemming from data scarcity and embodiment heterogeneity. To alleviate this, agents require robust embodied reasoning capabilities to connect the physical world with spatial concepts. We propose ``pointing'' as a unified, embodiment-agnostic representation to link observation with the decision, defining five core \textbf{E}mbodied \textbf{P}oint \textbf{R}easoning and Generation \textbf{A}bilities (\textbf{EPRA}). We first constructed EmbodiedPoints-200K datasets to enhance EPRA capabilities and introduce \textbf{Embodied-R1}, a VLM with powerful embodied reasoning capacity. Embodied-R1 is trained via a two-stage reinforcement learning process focusing on spatial reasoning and EPRA capabilities, thereby fostering powerful embodied reasoning abilities. It connects perception with environmental interaction through multiple pointing-centric signals to guide robotic decision-making for zero-shot manipulation. Extensive experiments across 11 benchmarks related to spatial understanding and EPRA comprehensively validate Embodied-R1's proficiency. With only 3B parameters, Embodied-R1 achieves state-of-the-art results on diverse benchmarks. Furthermore, its zero-shot capabilities in both simulated and real-world robotic manipulation show significant performance improvements over baseline methods, achieving a 45.9\% success rate in SimplerEnv and a 72\% success rate across 8 real-world tabletop manipulation tasks. 

Generalization in embodied AI is hindered by the ``seeing-to-doing gap'', stemming from data scarcity and embodiment heterogeneity. 
To address this, we pioneer ``pointing'' as a unified, embodiment-agnostic intermediate representation, defining four core embodied pointing abilities that bridge high-level vision-language comprehension with low-level action primitives. We introduce \textbf{\alg}, a 3B Vision-Language Model~(VLM) specifically designed for embodied reasoning and pointing. We use a wide range of embodied and general visual reasoning datasets as sources to construct a large-scale dataset, \textit{Embodied-Points-200K}, which supports key embodied pointing capabilities. Then we train \alg using a two-stage Reinforced Fine-tuning~(RFT) curriculum with specialized multi-task reward design. \alg achieves state-of-the-art performance on 11 embodied spatial and pointing benchmarks. Critically, it demonstrates robust zero-shot generalization by achieving a 56.2\% success rate in the SIMPLEREnv and 87.5\% across 8 real-world XArm tasks without any task-specific fine-tuning, representing a 62\% improvement over strong baselines. Furthermore, the model exhibits high robustness against diverse visual disturbances. Our work shows that a pointing-centric representation, combined with an RFT training paradigm, offers an effective and generalizable pathway to closing the perception-action gap in robotics.

\vspace{2mm}

\textit{Keywords: Embodied Reasoning, General Robotic Manipulation, Reinforcement Learning}

\vspace{5mm}

\coloremojicode{1F3E0} \textbf{Projects}: \href{https://embodied-r1.github.io/}{https://embodied-r1.github.io/}

\github{} \textbf{Code Repository}: \href{https://github.com/pickxiguapi/Embodied-R1}{https://github.com/pickxiguapi/Embodied-R1}

\coloremojicode{1F4DA} \textbf{Datasets}: \href{https://huggingface.co/collections/IffYuan/embodied-r1-684a8474b3a49210995f9081}{https://huggingface.co/IffYuan}

\coloremojicode{1F4E7} \textbf{Contact}: \href{mailto:yuanyf@tju.edu.cn}{yuanyf@tju.edu.cn}

\end{abstract}


==> sections/acknowledge.tex <==
\section{Acknowledgment}

We would like to thank Zhongwen Xu, Hongyao Tang, Liang Wang, Shuyang Gu, and Chen Li for their participation in the discussions of this paper and for providing valuable insights. In addition, we would especially like to thank Yiyang Huang for the constructive suggestions on improving the figures in the manuscript.

